Learning Depth Estimation for Transparent and Mirror Surfaces

Inferring the depth of transparent or mirror (ToM) surfaces represents a hard challenge for either sensors, algorithms, or deep networks. We propose a simple pipeline for learning to estimate depth properly for such surfaces with neural networks, without requiring any ground-truth annotation. We unveil how to obtain reliable pseudo labels by in-painting ToM objects in images and processing them with a monocular depth estimation model. These labels can be used to fine-tune existing monocular or stereo networks, to let them learn how to deal with ToM surfaces. Experimental results on the Booster dataset show the dramatic improvements enabled by our remarkably simple proposal.

==> table/stereo_generalization.tex <==

\begin{table*}[t]
\centering
\scalebox{0.55}{
\begin{tabular}{ccccc}
 & RAFT-Stereo \cite{lipson2021raft} && CREStereo \cite{li2022practical} \\\\
 % FULL RESOLUTION TABLES
 \begin{tabular}{ll}
 \toprule
 \\
 Category & Method \\
 \midrule
 \cellcolor{pink}All & Base \\
 \cellcolor{pink}All & Virtual Depth\\
 \cellcolor{pink}All & Merged  \\
% \cellcolor{pink}All & Merged Ft\\
 \bottomrule
 \toprule
 \cellcolor{blue!25}ToM & Base \\
 \cellcolor{blue!25}ToM & Virtual Depth\\
 \cellcolor{blue!25}ToM & Merged  \\
% \cellcolor{blue!25}ToM & Merged Ft\\
 \bottomrule
 \toprule
  \cellcolor{YellowOrange}Other & Base \\
 \cellcolor{YellowOrange}Other & Virtual Depth\\
 \cellcolor{YellowOrange}Other & Merged  \\
% \cellcolor{YellowOrange}Other & Merged Ft\\
 \bottomrule
 \end{tabular}
 &
 \begin{tabular}{rrrr | rr}
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px) & $\downarrow$ (px) \\
 \midrule
13.70 & 10.75 & 9.57 & 8.88 & 4.14 & 8.77 \\
\textbf{13.48} & \textbf{10.74} & 9.45 & 8.52 & 2.99 & 7.05 \\
15.16 & 11.46 & \textbf{9.30} & \textbf{7.71} & \textbf{2.10} & \textbf{4.85} \\
%14.75 & 10.87 & \textbf{8.65} & \textbf{7.03} & \textbf{1.98} & \textbf{4.53} \\

\bottomrule
 \toprule
\textbf{64.83} & \textbf{51.46} & \textbf{43.65} & \textbf{37.23} & 16.37 & 19.56 \\
65.29 & 56.46 & 50.12 & 45.51 & 15.02 & 17.74 \\
86.40 & 73.06 & 60.51 & 49.61 & \textbf{10.08} & \textbf{11.29} \\
%81.68 & 66.75 & 53.05 & 41.63 & \textbf{8.49} & \textbf{9.62} \\
\bottomrule
 \toprule
5.99 & 3.74 & 3.06 & 2.66 & 1.13 & 3.17 \\
\textbf{5.60} & \textbf{3.39} & \textbf{2.68} & \textbf{2.27} & \textbf{1.01} & \textbf{2.91} \\
6.01 & 3.76 & 3.08 & 2.68 & 1.13 & 3.17 \\
%6.01 & 3.76 & 3.08 & 2.67 & 1.13 & 3.16 \\
\bottomrule
 \end{tabular}
 & &
 \begin{tabular}{rrrr | rr}
 \toprule
 bad-2 & bad-4 & bad-6 & bad-8 & MAE & RMSE \\
 $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (\%) & $\downarrow$ (px) & $\downarrow$ (px) \\
 \midrule
12.35 & 9.25 & 7.97 & 7.24 & 3.07 & 6.90 \\
\textbf{11.31} & \textbf{7.98} & \textbf{6.49} & \textbf{5.57} & 2.52 & 4.86 \\
14.64 & 11.00 & 8.77 & 7.08 & \textbf{1.76} & \textbf{4.10} \\
%14.32 & 10.71 & 8.57 & 6.92 & \textbf{1.74} & \textbf{3.86} \\
\bottomrule
 \toprule
59.24 & 45.45 & 37.92 & 32.23 & 11.90 & 15.62 \\
\textbf{51.23} & \textbf{36.61} & \textbf{27.37} & \textbf{21.69} & \textbf{7.57} & \textbf{9.67} \\
85.70 & 72.03 & 58.36 & 48.14 & 9.59 & 10.82 \\
%81.17 & 65.64 & 51.88 & 40.93 & 8.20 & \textbf{9.32} \\
\bottomrule
 \toprule
6.14 & 3.87 & 3.11 & 2.66 & 0.94 & 2.39 \\
\textbf{5.27} & \textbf{3.04} & \textbf{2.33} & \textbf{1.92} & \textbf{0.78} & \textbf{2.24} \\
6.17 & 3.89 & 3.13 & 2.67 & 0.95 & 2.39 \\
%6.16 & 3.89 & 3.12 & 2.67 & 0.95 & 2.38 \\
\bottomrule
 \end{tabular}
 \end{tabular}
 }
 \caption{\textbf{Proxy Labels Stereo.}
 Generalization results on Booster train set at quarter resolution. All networks use the official weights released by authors. Best results in \textbf{bold}.}
 \label{tab:stereo_proxies}
\end{table*}


